Walk the Random Walk: Learning to Discover and Reach Goals Without Supervision

Learning a diverse set of skills by interacting with an environment without any external supervision is an important challenge. In particular, obtaining a goal-conditioned agent that can reach any given state is useful in many applications. We propose a novel method for training such a goal-conditioned agent without any external rewards or any domain knowledge. We use random walk to train a reachability network that predicts the similarity between two states. This reachability network is then used in building goal memory containing past observations that are diverse and well-balanced. Finally, we train a goal-conditioned policy network with goals sampled from the goal memory and reward it by the reachability network and the goal memory. All the components are kept updated throughout training as the agent discovers and learns new goals. We apply our method to a continuous control navigation and robotic manipulation tasks.

==> algo_long.tex <==

\begin{algorithm}[tb]
  \caption{Distance-based curriculum}
  \label{alg:method_long}
\begin{algorithmic}
    \State \textbf{Initialize:} $G_{train} = \{ s_0 \}$, replay buffer $\mathcal{R} = \{\}$, random trajectories buffer $\mathcal{T} = \{\}$
    \State \textbf{Input:} number of steps in episode $T$, number of episodes $N$, goals update interval $I_{goals}$, goals update threshold $\tau$
    \For{each episode}
        % \State
        % \State $s_0 = \texttt{env.reset()}$ 
        \State $g \gets \text{sample}(\mathcal{M})$ \Comment{Sample a goal from the memory}
        \For{each policy step}
            \State $a_t \sim \pi_\phi(s_{t-1}, g)$ \Comment{Sample an action from the policy}
            \State $s_t = \texttt{env.step}(a_t)$ \Comment{Act on the environment}
            \State $r_t = - d(s_t, g)$ \Comment{Reward by the distance function}
            \State $\mathcal{R} \leftarrow \mathcal{R} \cup \left\{ (s_{t-1}, s_t, a_t, r_t) \right\}$ \Comment{Store it in the replay buffer}
        \EndFor

        \State
        \State $\mathcal{T} \gets \emptyset$ \Comment{Collect a random trajectory}
        \For{each random step}
            \State $s_t \gets \texttt{env.step}(\text{random action})$
            \State $\mathcal{T} \gets \mathcal{T} \cup \{s_t\}$
        \EndFor
        \State $\mathcal{T} \gets \mathcal{T} \cup \{ \text{take T random steps} \}$
        \State
        \State $\phi \gets \text{policy.update}(R)$ \Comment{Update $\pi_\phi$ with SoftAC}
        % \State perform random steps and add trajectory to $\mathcal{T}$
        % \State $\mathcal{T} \gets \mathcal{T} \cup \{ \text{random steps} \}$
     \EndFor
     
     \State update $D$ with $\mathcal{T}$
     \State update $\mathcal{M}$

    \If {$n \equiv 0 \mod I_{goals}$}
        \For{every state $s$ in $\mathcal{T}$}
            \If {$d(s, G_{train}) > \tau$}
                \State $G_{train}$ = $G_{train} \cup \{s\}$
            \EndIf
        \EndFor
    \State $\mathcal{T} = \{\}$
    \EndIf
%   \IF {it is time to update $d$}
%   \STATE train $d$ on $\mathcal{T}$
%   \FOR{every state $s$ in $\mathcal{T}$}
%      \IF {$d(s, G_{train}) > \tau$}
%   \STATE add $s$ to $G_{train}$
%   \ENDIF
%   \ENDFOR
%   \STATE drop some trajectories from $\mathcal{T}$
%   \ENDIF
%   \STATE
\end{algorithmic}
\end{algorithm}


==> fig/maze4rooms_converge.tex <==
\begin{tikzpicture}[every node/.style={scale=0.8}]

% \footnotesize

\begin{axis}[
    width=7cm, height=5cm,
    ylabel = {distance to goal},
    xlabel = {policy training steps},
    grid=major,
    enlarge x limits=0,
    legend entries={Topline, $L_2$-curriculum, Our method},
    legend style={cells={anchor=west}},
]

% TOPLINE
\addplot+[
    cyan,
    mark=none,
] table [x=step,y=topline-mean]{fig/maze4rooms_converge.dat};

% ORACLE-CURRI
\addplot+[
    orange,
    mark=none,
] table [x=step,y=oracle-mean]{fig/maze4rooms_converge.dat};

% UNSUP
\addplot+[
    magenta,
    mark=none,
] table [x=step,y=unsup-mean]{fig/maze4rooms_converge.dat};

% TOPLINE ERR
\addplot[
    name path=upper,
    draw=none,
] table [x=step,y expr=\thisrow{topline-mean}+\thisrow{topline-std}]
    {fig/maze4rooms_converge.dat};
\addplot[
    name path=lower,
    draw=none,
] table [x=step,y expr=\thisrow{topline-mean}-\thisrow{topline-std}]
    {fig/maze4rooms_converge.dat};
\addplot [fill=cyan, fill opacity=0.1] fill between[of=upper and lower];

% CURRI ERR
\addplot[
    name path=upper,
    draw=none,
] table [x=step,y expr=\thisrow{oracle-mean}+\thisrow{oracle-std}]
    {fig/maze4rooms_converge.dat};
\addplot[
    name path=lower,
    draw=none,
] table [x=step,y expr=\thisrow{oracle-mean}-\thisrow{oracle-std}]
    {fig/maze4rooms_converge.dat};
\addplot [fill=orange, fill opacity=0.1] fill between[of=upper and lower];

% UNSUP ERR
\addplot[
    name path=upper,
    draw=none,
] table [x=step,y expr=\thisrow{unsup-mean}+\thisrow{unsup-std}]
    {fig/maze4rooms_converge.dat};
\addplot[
    name path=lower,
    draw=none,
] table [x=step,y expr=\thisrow{unsup-mean}-\thisrow{unsup-std}]
    {fig/maze4rooms_converge.dat};
\addplot [fill=magenta, fill opacity=0.1] fill between[of=upper and lower];

\end{axis}

\end{tikzpicture}
